Robust Deep Reinforcement Learning for Extractive Legal Summarization

Automatic summarization of legal texts is an important and still a challenging task since legal documents are often long and complicated with unusual structures and styles. Recent advances of deep models trained end-to-end with differentiable losses can well-summarize natural text, yet when applied to legal domain, they show limited results. In this paper, we propose to use reinforcement learning to train current deep summarization models to improve their performance on the legal domain. To this end, we adopt proximal policy optimization methods and introduce novel reward functions that encourage the generation of candidate summaries satisfying both lexical and semantic criteria. We apply our method to training different summarization backbones and observe a consistent and significant performance gain across 3 public legal datasets.

==> cut.tex <==
\begin{algorithm}[ht]
\caption{Algorithm for Keyword Reward}
\label{algo:kw}
\begin{algorithmic}[1]
\Require {A document: $D$, a summary: $S$, Number of keywords:$n_k$;}
\Ensure {Keyword rewards $R_{kw}$;}
\Function{Get\_Keywords}{Text: $T$, Number of keywords:$n$}
% \State $U \leftarrow \emptyset$
% \For{$phrase \in T$}
%     \State Add $(phrase, \|emb(phrase) \|)$ to $U$
% \EndFor
% \State Sort U by its second values
% \State $initial\_set \leftarrow \{v: v \in U[i] \land i \leq 2 * n \}$ {\scriptsize\it Get top $2*n$ keywords from U}
\State $U \leftarrow$ Top $2*n$ keywords from $T$ {\scriptsize\it Based on $ \|emb(phrase)\|$ }
\State $S \leftarrow initial\_set[1]$ %{\scriptsize\it Create a final set containing only the first keyword of the initial set}
\While {$|S| < n$}
    % \State $best\_value \leftarrow 1$
    % \For {$k \in initial\_set \setminus	final\_set$} {\scriptsize\it Find the least similarity keyword compared to $final\_set$}
    %     \State $most\_sim \leftarrow \max_{k' \in final\_set} (cosine\_sim(k,k'))$
    %     \If {$most\_sim < best\_value $}
    %         \State $best\_k \leftarrow k$
    %     \EndIf
    % \EndFor
    %\State $best\_k \leftarrow \argmin_{k \in initial\_set \setminus	final\_set} \left( \max_{k' \in final\_set} cosine\_sim(k,k') \right)$
    \State $best\_k \leftarrow $ The least similarity keyword compared to $S$
    \State Add $best\_k$  to $S$
\EndWhile
\State Return $S$;
\EndFunction
\State $kw(D) \leftarrow Get\_Keywords(D,n)$
\State $kw(S) \leftarrow Get\_Keywords(S,n)$
\State $A \leftarrow \emptyset$
\For{$k \in kw(D)$}
    \State Add $max_{k' \in kw(S)} consine(k,k')$ to A
\EndFor
\State Return $Average(A)$; 
\end{algorithmic}
\end{algorithm}


==> discuss.tex <==
 
